Dense matter with eXTP

In this White Paper we present the potential of the Enhanced X-ray Timing and Polarimetry (eXTP) mission for determining the nature of dense matter; neutron star cores host an extreme density regime which cannot be replicated in a terrestrial laboratory. The tightest statistical constraints on the dense matter equation of state will come from pulse profile modelling of accretion-powered pulsars, burst oscillation sources, and rotation-powered pulsars. Additional constraints will derive from spin measurements, burst spectra, and properties of the accretion flows in the vicinity of the neutron star. Under development by an international Consortium led by the Institute of High Energy Physics of the Chinese Academy of Science, the eXTP mission is expected to be launched in the mid 2020s.

==> dotar <==
tar cvf eXTP_WP_OS.tar \
2017SCGE.cls                    \
BB_1mCrab_ld_del_eemo_jz.eps	\
Clump.eps			\
collision.eps			\
dotar				\
elavsky4.png			\
eXTP_CV_fig.eps			\
extp.eps			\
eXTP_WP_OS.tex		\
facilities_vs9jan2018.pdf	\
famps_extp7.eps			\
figgrb1_vs6.eps			\
figgrb2b.pdf			\
figgrb3_vs3.eps			\
figgrbiron1_vs2.eps		\
figgrbiron2_vs2.eps		\
FoV_vs26092017.pdf		\
jean4m2.pdf			\
lc_extp5.eps			\
lmxb_orbitsn.pdf		\
LOFT_AGN_var_totcounts.pdf	\
patruno.png			\
radiomap3.eps			\
sens.pdf			\
snr1.eps			\
spectra.eps			\
stellarflare_artist.eps		\
v0332_crit.pdf                  \
wu2010.png                      \
picins.sty                      \
Print-CrossMark.eps                  \
Print-CrossMark-eps-converted-to.pdf \
figDrake3b.eps                       \
sn1006_1_srcut_sfa_1e4.eps           \
eXTP_WP_OS.pdf

gzip eXTP_WP_OS.tar

